Atomic source selection in space-borne gravitational wave detection

Recent proposals for space-borne gravitational wave detectors based on atom interferometry rely on extremely narrow single-photon transition lines as featured by alkaline-earth metals or atomic species with similar electronic configuration. Despite their similarity, these species differ in key parameters such as abundance of isotopes, atomic flux, density and temperature regimes, achievable expansion rates, density limitations set by interactions, as well as technological and operational requirements. In this study, we compare viable candidates for gravitational wave detection with atom interferometry, contrast the most promising atomic species, identify the relevant technological milestones and investigate potential source concepts towards a future gravitational wave detector in space.

==> tables/dkc_estimations.tex <==
% DEPRECATED

\begin{table}
\centering
\begin{tabular}{l|cc|cc} 
\multirow{2}{*}{3D expansion rate $T = 10$\,pK} & \multicolumn{2}{c|}{Collisionless}&\multicolumn{2}{c}{Hydrodynamic}\\[5pt]
 & $^{174}$Yb & $^{84}$Sr & $^{174}$Yb & $^{84}$Sr \\ 
 \hline\hline
\rule{0pt}{2.6ex}Number of atoms &\multicolumn{2}{c|}{$5\times 10^8$} & \multicolumn{2}{c}{$5\times 10^7$} \\[1pt]
Trapping frequency \hfill [2$\pi$ Hz]	 & \multicolumn{2}{c|}{25}  & \multicolumn{2}{c}{50}  \\[1pt]
Initial temperature \hfill [$\mu$K]& \multicolumn{2}{c|}{10} & \multicolumn{2}{c}{0.83}  \\[1pt]
Initial size	$2 \sigma_0$ \hfill [$\mu$m]	& 393.77 & 566.91 & 58.03 & 83.22 \\[1pt]
\hline
\rule{0pt}{2.6ex}Knudsen parameter & 0.28 & 0.42 & 0.06 & 0.09 \\[1pt]
Phase space density	& \multicolumn{2}{c|}{$<10^{-3}$} &\multicolumn{2}{c}{0.6} \\[1pt]
\hline
\rule{0pt}{2.6ex}Pre-DKC  expansion time ($t_-$) \hfill [ms]& \multicolumn{2}{c|}{6359} & \multicolumn{2}{c}{924} \\[1pt] 
Size at lens $2\sigma(t_-)$\hfill [mm] 	& \textbf{393.32} &  \textbf{566.27} & \textbf{ 16.73 }&\textbf{ 23.99 }\\[1pt]
Final size	$2\sigma(t_-+2T$) \hfill [mm] &   &   &   &   \\[1pt]
\hspace{1cm} T=40s						& 393.34 & 566.29 & 17.09 & 24.51 \\[1pt]
\hspace{1cm} T=100s					& 393.42 & 566.41 & 18.88 & 27.09 \\[1pt]
\hspace{1cm} T=160s					& 393.57 & 566.63 & 21.81 & 31.33 \\[1pt]
\end{tabular} 
\caption{DKC performance for classical gases.}
\label{tbl:dkcperf1}
\end{table}

\begin{table}
\centering
\begin{tabular}{l|cc|cc} 
\multirow{2}{*}{3D expansion rate $T = 10$\,pK} & \multicolumn{2}{c|}{BEC}&\multicolumn{2}{c}{DFG}\\[5pt]
 & $^{174}$Yb & $^{84}$Sr & $^{171}$Yb & $^{87}$Sr \\ 
 \hline\hline
\rule{0pt}{2.6ex}Number of atoms &\multicolumn{2}{c|}{$7\times 10^6$} & \multicolumn{2}{c}{$7\times10^6$} \\[1pt]
Trapping frequency \hfill [2$\pi$ Hz]	 & \multicolumn{2}{c|}{50}  & \multicolumn{2}{c}{50}  \\[1pt]
Critical temperature \hfill [$\mu$K]& \multicolumn{2}{c|}{0.431} & \multicolumn{2}{c}{0.834}  \\[1pt]
Initial size	 $2 R_0$ \hfill [$\mu$m]	& 30.2 & 41.8 & 56.86 & 81.86 \\[1pt]
\hline
\rule{0pt}{2.6ex}Pre-DKC  expansion time ($t_-$) \hfill [ms]& 63 & 61 & 460 & 460 \\[1pt] 
Size at lens $2R(t_-) $\hfill [mm] 	& \textbf{0.50}&\textbf{0.67}& \textbf{8.21}& \textbf{11.82}\\[1pt]
Final size	$2R(t_-+2T$) \hfill [mm] &   &   &   &   \\[1pt]
\hspace{1cm} T=40s							&  9.27 &  13.34 &  12.86 & 18.51 \\[1pt]
\hspace{1cm} T=100s						&  23.15 & 33.32 & 26.07 & 37.53 \\[1pt]
\hspace{1cm} T=160s						& 37.03 & 53.31 & 40.43 & 58.20 \\[1pt]
\end{tabular}
\caption{DKC performance for degenerate gases.} 
\label{tbl:dkcperf2}
\end{table}

==> tables/quenching.tex <==
\begin{center}
\lineup
\begin{tabularx}{\linewidth}{l*{6}{Y}}
\toprule
 Regime & \multicolumn{2}{c}{Thermal} & \multicolumn{2}{c}{Hydrodynamic} & \multicolumn{2}{c}{BEC}\\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
Atomic species  &  \textsuperscript{174}Yb  &  \textsuperscript{84}Sr & \textsuperscript{174}Yb  &  \textsuperscript{84}Sr &  \textsuperscript{174}Yb       &      \textsuperscript{84}Sr \\
Atom number & \multicolumn{2}{c}{\SI{5e8}{}} & \multicolumn{2}{c}{\SI{5e7}{}} & \multicolumn{2}{c}{\SI{7e6}{}} \\
Transverse temp. (pK) & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{10} \\
Effective linewidth (\SI{}{\nano Hz/2\pi}) & 855 & 460 & 855 & 460 & 855 & 460\\
  Ensemble radius (mm)  &  394 &  567 &  21.8  &  31.3  &  14.0  &  20.2 \\
  Rabi frequency (\SI{}{Hz/2\pi})  &  \textcolor{red}{0.04}  &  \textcolor{red}{0.03}  &  \textcolor{red}{0.7}  &  \textcolor{red}{0.5}  &  \textcolor{red}{1.1}  &  \textcolor{red}{0.8} \\
\bottomrule
\end{tabularx}
\end{center}
